Harder, better, faster, stronger: understanding and improving the tractability of large energy system models

Energy system models based on linear programming have been growing in size with the increasing need to model renewables with high spatial and temporal detail. Larger models lead to high computational requirements. Furthermore, seemingly small changes in a model can lead to drastic differences in runtime. Here, we investigate measures to address this issue. We review the mathematical structure of a typical energy system model, and discuss issues of sparsity, degeneracy and large numerical range. We introduce and test a method to automatically scale models to improve numerical range. We test this method as well as tweaks to model formulation and solver preferences, finding that adjustments can have a substantial impact on runtime. In particular, the barrier method without crossover can be very fast, but affects the structure of the resulting optimal solution. We conclude with a range of recommendations for energy system modellers.

==> background.tex <==

\section{Background} \label{sec_background}

We first give a high-level overview of the structure of a typical energy system model as a network flow model, using its implementation in the Calliope modelling software \cite{Pfenninger2018} as an example. We then proceed to discuss the resulting optimisation problem, its properties, and how these have been treated in existing literature. Finally, we examine how scaling issues in such problems have been treated so far, given that improved scaling seems to have particularly high potential for improving solution speed and accuracy.

\subsection{Energy system models as network flow models} 

A high-level view of the problem we want to solve is the following: Given geographically distributed consumers and producers of "goods" such as electricity or heat (from now on referred to as \texttt{carriers}) and a network over which these carriers can be transferred we want to find the cheapest way to allocate these carriers over time and between locations such that all demand for them is covered. In other words, we want to solve a minimum-cost flow problem with multiple commodities. \mb{Maybe add the formulation of min-cost flow problem here s.t. the link to LP is clearer or at least cite an authoritative source that explains it} \sjp{Manuel: can we just cite an authoritative source on the min-cost flow problem here?}

The most basic component of our model is a \texttt{technology}, of which we have five basic kinds. Supply technologies convert a resource form outside the model boundary (e.g. sunlight) into a carrier (e.g. electricity). The resource is often limited and time dependent (given as a time series). Demand technologies consume a certain amount of a carrier, usually specified in a time series. Storage technologies allow storing a carrier and reusing it later, transmission technologies allow sending carriers between locations, and conversion technologies allow converting one carrier into another (e.g. electricity to heat). All of these with the exception of demand perform a transformation: between location, time, or carrier; these transformations are limited by a certain capacity and incur a cost.

\definecolor{supply}{HTML}{559bda}
\definecolor{conversion}{HTML}{78d08b}
\definecolor{demand}{HTML}{f4b557}
\definecolor{storage}{HTML}{ff9999}
\definecolor{transmission}{HTML}{8d44c7}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \resizebox{.95\linewidth}{!}{
            \input{figures/flow.tex}
        }
        \caption{A simple model with three locations and their technologies: \textcolor{supply}{supply}, \textcolor{demand}{demand}, \textcolor{storage}{storage}, \textcolor{conversion}{conversion} and \textcolor{transmission}{transmission}. }
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \resizebox{.95\linewidth}{!}{
            \input{figures/flow_abstract.tex}
        }
        \caption{Formulation as network flow problem considering $2$ timesteps. Each edge has associated capacity and cost (not depicted here for legibility).}
    \end{subfigure}
    \caption{The general structure of a simple energy system model formulated with Calliope.}
    \label{fig:model}
\end{figure*}


Figure \ref{fig:model} shows an example model. We can translate many of the features of such an energy model into the language of network flow problems. Resource demand/supply can be modelled as edges from/to a designated source/sink with the given capacity. The transformation performed by technologies can be modelled as edges that have both cost and capacity. Choosing the source and destination nodes as representing either different locations, different timesteps, or carriers, we can model transformations in space, time and type of carrier respectively. Separate timesteps can be modelled as multiple copies of a static model where some components of those model copies are linked together (Figure \ref{fig:model}.b).

Using these standard modelling techniques we can translate the model of Figure \ref{fig:model} into the network flow model depicted in Figure \ref{fig:flow} and the problem then reduces to finding a minimum cost flow that satisfies the demands of all nodes.

However, there are two major problems when trying to model real energy models as flow problems. First, modelling the transformations described above as edges with capacity and cost neglects the fact that most transformations have a certain \texttt{efficiency} associated with them. For example it is not possible to store energy in a battery without loss. These efficiencies are usually modelled as multiplicative factors. It seems impossible to incorporate this in a network flow model. Second, energy models are usually set up to include some additional constraints to reflect certain policy or planning restrictions, e.g. limiting production by non-renewable energy sources. In Calliope we refer to the implementation of such policies as \texttt{group constraints}, as they effect groups of locations, technologies, or carriers. In terms of a network flow model a general group constraint prescribes upper or lower bounds on the cumulative flow through a set of edges. Depending on the exact formulation of the problem some kinds of group constraints may be possible to represent \mb{but this is probably not possible in general? The simplest example that seems impossible to model is the following: restrict the cumulative output of two coal plants with different efficacy. There are two things (right?) one could try: limit the cumulative inputs (resource) of both plants or limit the cumulative outputs (carriers) of both plants. In the first case one has the problem that different efficacies makes it impossible to set the limited input correctly. In the second case a "limiting" node would need to aggregate the outputs of the plants in the group. But such a limiting node would make it impossible to represent the correct transmission lines from each plant to other nodes }.

Given the deficiencies of the flow model we now turn to the more expressive model of linear programs. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% previously existing content begins:

% \textit{An abstract diagrammatic view of what an energy system model does – using Calliope terminology and Calliope techs with a few locations.}

% At its most basic, it’s a network flow model. \textit{Show a diagram of that.} We need to understand how one would deal with a generic network flow model more effectively and whether there’s something to apply there – just to mention it, while in practice we think most models will need group constraints and stuff like that. But we think it could still be interesting to talk about briefly.

% BUT the following properties force us to model the problem using the more general class of LP problems:
% \begin{itemize}
% 	\item We have conversion techs: that means we link two network flow models
% 	\item We have storage techs: we connect timesteps – but we connect only adjacent ones so that should be better than connecting distant ones
% 	\item We have group constraints: they destroy any structure in the network flow problem that would allow nice methods to be used.
% \end{itemize}

% previously existing content ends
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Linear optimisation of network flow models}
\label{subsec_mathematical}

The general form of an LP is
\begin{align} \label{eq:lp}
\begin{split}
    \text{minimize}\ &c^\intercal x \\
    \text{s.t.}\ &Ax = b \\
    &l \leq x \leq u
\end{split}
\end{align}
For $A \in \mathbb{R}^{n\times m}, b \in \mathbb{R}^m, c, l, u \in \mathbb{R}^n$. We refer to $A$ as the constraint matrix, to $c$ as the objective and to $l$ and $u$ as lower and upper bounds of $x$ respectively. Formulating a minimum-cost flow problem as an LP is straightforward:
$x_i$ is the variable holding the amount of flow through the $i$-th edge. $l_i$ and $u_i$ limit the capacity of the $i$-th edge. Row $j$ of $A$ contains a non-zero entry at index $i$ which is $1$ or $-1$ if the $i$-th edge is an incoming or outgoing edge of node $j$ respectively. $b_j$ is the flow-demand of node $j$. $c_i$ is the cost incurred by one unit of flow at edge $i$. 

Additionally, the LP formulation allows for convenient representation of \textit{efficiencies} and \textit{group constraints}. A constraint requiring the sum over all inputs of a technology to be equal to some factor $f \in (0,1]$ times all outputs of that technology asserts an efficiency of $f$ of that technology. Similarly, a group constraint is just a bound on the sum of the inputs or outputs of several technologies.

The authors of \cite{ref_parallel_ip} observe that the constraint matrix of energy system LPs naturally have an \texttt{arrowhead} structure as depicted below:
\begin{center}
\input{figures/matrix}
\end{center}
Where non-zero entries are marked gray. This non-zero pattern visualizes a relationship between constraints or variables that is inherent in ESMs: due to the time-discrete nature of ESMs many variables are specific to a certain timestep, and on the other hand, many constraints affect only a certain timestep. For example, the rows intersecting $\tau_1$ are constraints that  affect only variables $x_1$, part of $x_2$ and $x_3$. Similarly variables $x_2$ are further only affected by rows touching $c_1$ and $c$. 

\subsubsection{Solving linear programs} \label{sec_solving_lp}
The two most widely used families of algorithms used to solve linear programs are simplex methods and barrier methods. Many variants of these methods exist and there are detailed sources for most of them but for our purposes the compact overview of the revised primal-simplex method and Dikin’s Primal Affine Scaling Algorithm (as an example of a barrier method) as provided in section 2 of \cite{guidelines_klotz} suffices. Neither of the two families of methods is generally faster than the other. Instead what algorithm should be used depends on the structure of the LP at hand \cite{Tomlin1989, guidelines_klotz}.

An important distinction between simplex and barrier methods is that the former always returns a basic feasible solution (we will call this either BFS or a vertex solution, depending on the contex) if an optimal solution exists at all, whereas the latter generally returns an interior point that is close enough to optimal (we call this a midface solution). Given a midface solution as returned by the barrier method, the crossover method can be performed to find a BFS \cite{ref_recovering_basis_bixby}. A BFS may be preferable to a midface solution for several reasons as discussed in Section \ref{subsection_results_useful_but}, in particular a BFS is \textit{needed} for further processing if the problem is a mixed-integer linear program (MILP).

\subsubsection{Properties of ESMs as linear programs} \label{sec_properties}
We now consider several properties of ESMs as LPs and the consequences of these properties. 
\begin{enumerate}
    \item The problems are highly sparse: note that the number of zero entries scales quadratically in the number of timesteps, whereas the number of nonzero entries is linear in the number of timesteps.
    \item Standard minimum-cost flow problems are often inherently degenerate \cite{network_flows, Tomlin1989}. Degeneracy in the context of linear programming means that multiple bases of the constraint matrix $A$ lead to the same basic feasible solution. Degeneracy can cause an increased runtime for some solution algorithms, in particular for the Simplex algorithm (c.f. below). In the context of network-flow problems degeneracy means that a rerouting of the flow (usually in the context of a pivot operation of the Simplex method) fails to decrease the cost of the flow. \mb{Our LPs differ from standard minimum-cost flow problems by imposing additional constraints on the flow: explain why this is still an issue...}
    
    %In the LP formulation of a minimum-cost flow problem, a basis of the constraint matrix $A$ corresponds to a subset of the edges $B \subseteq E$ (in particular $B$ is a spanning tree of the network \cite{network_flows}). In a basic feasible solution the flow $x_i$ of an edge $e_i \in E \setminus B$ is at either at its upper bound $u_i$ or at its lower bound $l_i$ and the flows $x_j$ of edges $e_j \in B$ are then chosen such that the demands $b$ of all nodes are met. A basic feasible solution is thus degenerate if for some basic edge $e_i \in B$ it holds that its flow $x_i$ is at its bound $x_i \in \{l_i, u_i\}$.
    \item The problems often have large numeric ranges. This is a consequence of the fact that the entries of $A$ represent quantities of different physical units (e.g. energy, area, cost). 
    \item ESMs have a useful interpretation of infeasibility: the energy demand cannot be satisfied given the means of production. In these cases an infeasibility certificate is often not satisfactory for the modeller who may nevertheless wish to investigate the optimal resource allocation. Such models can be forced to be feasible by what is known in general as the Big-M method: in the context of ESMs this means that we associate a cost factor with units of unmet demand. In order for the optimal solution to have unmet demand only if necessary, this associated cost has to be huge. The Big-M method thus is another factor that causes large numeric ranges in the model. 
\end{enumerate}
In the following we want to consider how the above mentioned properties may affect the performance of simplex style and barrier methods.

\paragraph{sparsity}
Simplex and Barrier both have ways of profiting from sparsity in the constraint matrix $A$. Simplex uses Markowitz pivoting and permutation (factor out the usually large part of the matrix that is triangular) to produce a very sparse LU-decomposition of $A$ that allows quick computation of the pivot operation \cite{suhl_suhl_90, suhl_suhl_93, sparse_lu}. Barrier uses fast Cholesky factorization methods to factor symmetric matrices containing $AA^\intercal$ in each step. These factorizations of barrier are more amenable to parallelization than the computations involved in simplex pivoting \cite{guidelines_klotz}. Moreover, recent advances have been made to further exploit parallelism in the barrier method for the special case ESMs by exploiting their inherent block-structure \cite{ref_parallel_ip}.

Barrier performs a very small amount of iterations (empirical magic number of around 50-100, almost independent of problem size \cite{beam_me}) that are very costly. Simplex performs very many steps (some people suggest around $2m$ on average \cite{Tomlin1989}), but each step is quite cheap. The authors of \cite{guidelines_klotz} provide some guidelines on how to choose the solution method based on structural properties of the problem. In particular they observe that the barrier method may not be suitable for problems with many dense columns because dense columns lead to $AA^\intercal$ being dense too, whereas dense rows do not.

\paragraph{Degeneracy}
Degeneracy can either be an artifact of the way a problem is formulated (structural degeneracy) or it can be inherent in the problem (inherent degeneracy). While structural degeneracy can be dealt with in parts in a preprocessing step called presolve, the same is not true for inherent degeneracy \cite{presolve, Tomlin1989}. As stated before, our problems are inherently degenerate and this has consequences on how they should be solved:

The simplex method finds a solution to the linear program by jumping from one basic feasible solution to the next. For the simplex method degeneracy thus means that pivot steps may lead to no improvement of the objective. Computational studies have shown that applying the simplex method directly to min-cost flow problems may not work well because a fraction of up to 90\% of all pivot operations can be degenerate \cite{network_flows}. A specialized implementation of the simplex method for network-flow problems exists that can avoid degenerate steps by exploiting graph theoretic properties of the basic feasible solutions \cite{network_flows}. However, the network simplex algorithm works on an explicit graph and thus cannot be applied in our setting as we rely on a constraint matrix $A$. 

Barrier methods, however, maintain an interior point of the feasible region and never actually encounter a basic feasible solution until the very end, when optimality is reached. Degeneracy thus has no effect on the efficacy of interior-point methods \cite{guidelines_klotz}.
\mb{we don't have results about degeneracy... except maybe that barrier is a lot better than simplex... keep this?}

\paragraph{Parameter range}
To understand the relevance of the parameter range for the solution of a linear program, we have to introduce the notion of the condition number of a matrix.
The condition number of a matrix $A$ is defined as 
\[
\kappa(A) = \max_{\lVert v \rVert, \lVert w \rVert = 1} \frac{\lVert A^{-1} v \rVert}{ \lVert A^{-1} w \rVert}
\]
and can be interpreted as the maximal effect disturbing the rhs $b$ has on the solution $x$ of the LSE $Ax = b$. A matrix is called ill-conditioned if $\kappa$ is large. An ill-conditioned matrix has the problem that the computation of its inverse and thus also of the solution of its linear system of equations is prone to large numerical errors.

Simplex style and barrier methods both rely on the solution of linear systems of equations involving parts of $A$ in every step. Thus the success of both families of algorithms depends on the condition number of the encountered matrices. However, the exact relationship between the condition number of $A$ and the condition number of the matrices encountered throughout the algorithm is complicated \cite{ref_scaling_12}. Condition number and parameter range of a matrix are tightly related and several authors have studied this relationship \cite{algo_d, algo_sigma}. We will discuss this relationship and ways of handling large numerical ranges in section \ref{subsec_scaling}

\paragraph{Big-M}
It is well known \mb{maybe need a citation for this} that large constants used in the big-M method can prevent the solution method from converging. Moreover, \cite{beam_me} observes that the solution time of otherwise identical ESMs scale with increasing big-M constant. It is therefore advisable to choose the big-M constant as small as possible. In general we want to associate a cost $M$ with one unit of unmet demand, such that the following property holds

\begin{align} \label{big_m}
\begin{split} 
  \text{unmet demand} = c > 0 \Longrightarrow &\text{ the allocation problem is infeasible} \\
  &\text{and exactly c units of demand cannot} \\
  &\text{be satisfied}
  \end{split}
\end{align}

We want to choose M as small as possible such that (\ref{big_m}) holds. Note that if a node (in the abstract min-cost flow model sense) has one unit of unsatisfied demand, it will satisfy this demand from "unmet demand" only if there is either no other way to satisfy it, or if the cost c is smaller or equal the cost of satisfying the demand otherwise. Thus in order to ensure condition (\ref{big_m}) we need to choose M larger than the maximum possible cost of one unit of any demand-carrier.
\mb{we don't have results about bigM... remove?}

\vspace{20pt}
In section \ref{subsec_methods} we will try to answer the question if either the simplex or the barrier method is more favorable to solve ESMs given the inherent degeneracy, sparsity, and other structural properties of these LPs. In order to do this we conduct a series of benchmarks using a range of Calliope models. The problem of large numerical ranges will be more thoroughly discussed in section \ref{sec_scaling}. We further propose a scaling algorithm that may alleviate the problem of large numerical ranges and test the effectiveness of this algorithm with a series of benchmarks in section \ref{subsec_methods}. 

\subsection{Scaling of Linear Programs} \label{sec_scaling}
\mb{could remove this and cite \cite{ref_scaling_93} who includes something similar}
As discussed in Section \ref{subsec_mathematical}, a large numeric range of the constraint matrix $A$ can have a bad impact on the solution time of the optimization problem. The problem of large numeric ranges can sometimes be alleviated by scaling rows and columns of $A$. We now first argue why and how we can freely scale rows and columns of an LP constraint matrix $A$. Let us denote by $R$ and $S$ two diagonal matrices 
\[
R = \mathbf{diag}(r_1, \dots, r_n), \qquad S = \mathbf{diag}(s_1, \dots, s_n)
\]
with $r_i, s_i > 0$. Furthermore, let $A \in \mathbb{R}^{m \times n}$, $b \in \mathbb{R}^m$ and $c \in \mathbb{R}^n$. Let's consider the three polytopes $P := \{x\ |\ A x \leq b\}$, $P'' := \{x\ |\ RAx \leq Rb\}$ and $P' := \{x\ | RASx \leq Rb\}$.  then the following two LPs are equivalent
\begin{align*}
&\min c^\intercal x   &   &\min c^\intercal S x  \\   
&\text{s.t. } x \in P  &    &\text{s.t. } x \in P'    
\end{align*}
To see this note that $P = P''$ because $R$ is invertible and that for each $x \in \mathbb{R}^n$ holds $x \in P' \Leftrightarrow Sx \in P''$. The scaled LP instance might, however, have much better numerical properties. We can choose arbitrary row/col-scaling factors $r_i, s_i > 0$ and try to improve these numerical properties.


\subsubsection{Effects of scaling on solving LPs} \label{subsec_scaling}
The effect of scaling on solving LPs is badly understood from a theoretical point of view \cite{ref_scaling_12}. A common approach of investigating scaling methods is via computational tests. Many authors have tested the effectiveness of various scaling algorithms on a set of LP problems with respect to (a subset of) the following metrics \cite{ref_scaling_75, ref_scaling_93, ref_scaling_12, ref_scaling_13}
\begin{enumerate}          
	\item The condition number of the scaled constraint matrix $A$
	\item The condition number of the bases of $A$ encountered during the simplex algorithm
	\item The number of simplex iterations required to solve the scaled LP
	\item The total runtime to solve the scaled LP
	\item The numerical behavior of the algorithm
\end{enumerate}


\paragraph*{Effect of scaling on the simplex method}
The most extensive computational test of this type that we are aware of was performed by \cite{ref_scaling_12} where they investigated a large number of scaling techniques and their effect on a large number of real world LPs. However, they only considered the simplex method.

\cite{ref_scaling_12} observes that the larger the condition number $\kappa$ of a basis of the constraint matrix $A$ the 'flatter' is the corresponding vertex of the polyhedron. Very flat corners are undesirable because they limit the amount of progress we can make by a simplex step. However, \cite{ref_scaling_12} further observes that a priori we can only minimize $\kappa$ of the whole constraint matrix and not exclusively of the bases encountered during the simplex algorithm. In particular minimizing $\kappa(A)$ may increase $\kappa$ of all relevant bases of $A$ and thus increase the runtime of the simplex algorithm.

The computational results in \cite{ref_scaling_12} can be summarized as follows (with respect to the metrics listed above)
\begin{enumerate}
	\item scaling can cause an increase in the average condition number of the square basis matrices B encountered in the simplex algorithm
	\item on average none of the scaling algorithms proposed to date is able to reduce the number of required simplex iterations.
	\item scaling is able to provide a reference point for the magnitude of absolute tolerances
\end{enumerate}
To (3) it is worth noting that the Gurobi documentation similarly states that scaling should be applied to ensure that all values are at most on the order of $10^4$ for them to work well with the absolute tolerances used in Gurobi.

\paragraph*{Effects of scaling on interior-point methods}
\cite{ref_scaling_13} Conduct a smaller study only considering arithmetic mean, geometric mean and equilibration scaling techniques. Moreover, they only consider randomly generated LPs. They don't mention how exactly they generate these matrices (meaning that we don't know how relevant the considered LP instances are in practice. \cite{ref_scaling_12} states that it is well understood that Gaussian random constraint matrices are unlikely to have any ill-conditioned bases). However, they investigate their effect on an interior point method solver which is more relevant to our use case. They conclude that equilibration scaling is the best among the three scaling techniques they consider and that it is most useful for the IPM solver (compared to simplex style and exterior point). They conclude that scaling on IPM achieves to reduce noticeably (2x to 3x) both the solution time and the number of iterations needed by the algorithms.

\paragraph{Effects of scaling on Crossover}
\mb{maybe leave this out? Or cut it down to the bit explaining markowitz pivoting}
To the best of our knowledge no author explicitly discusses the effects of scaling on crossover \mb{Note: this may be discussed partially in Meggido's paper on optimal basis construction... check!}. In this section we will argue that large numerical ranges may adversely affect the success and speed of crossover.

\mb{Caveat: this section is based on the description of the crossover algorithm described in \cite{ref_recovering_basis_bixby}. This is not necessarily exactly the same algorithm as the one applied in Gurobi, but I think the general ideas will be the same.}

After the actual interior point method has returned an optimal solution $x_{\text{IP}}^*$ we apply the crossover method in order to get a basic feasible solution $x^*$, meaning a \textbf{vertex} of the polyhedron achieving the same objective value as $x_{\text{IP}}^*$. Roughly speaking, crossover consists of the following two steps
\begin{enumerate}
	\item Choose a vertex $x$ close to $x_{\text{IP}}^*$. This amounts to choosing a basis $B$ (set of $n$ row and col indices yielding a square submatrix of $A$ with full rank)  that satisfies $A_B x_B = b' \approx b$.
	\item Do simplex steps from this basis $B$ until an optimal vertex is found
\end{enumerate}
How quickly this can be done depends mainly on two things: 
\begin{enumerate}
	\item how fast can such a basis $B$ be constructed
	\item how many simplex steps are necessary to arrive from $B$ at an optimal vertex
\end{enumerate}
It turns out that both are related to how well conditioned $A$ is: columns of $A$ for which no acceptably large (in absolute value) pivot entry can be found, won't be included in the basis \cite{ref_recovering_basis_bixby}. Meaning that if $A$ is ill-conditioned, potentially many desirable variables won't be included in the initial basis $B$ which then may necessitate more simplex iterations in step 2. 

Moreover, the algorithm chooses a basis by considering columns of $A$ in the order of 'desirability' and tries to generate a well-conditioned matrix from the most 'desirable' columns first. If many columns need to be discarded this means that the search for a suitable pivot-element must be repeated for many columns of $A$ \cite{ref_recovering_basis_bixby}.

Furthermore, the construction of basis $B$ even needs to be restarted if the resulting basic solution $x := A_B^{-1} b$ features too large infeasibilities. Crossover is then tried again with an increased threshold value for pivot elements, often referred to as Markowitz tolerance \cite{ref_recovering_basis_bixby}.

\subsubsection{Metrics \& goals of scaling}
In general there is little consent on how much good scaling can do: On the one hand \cite{ref_scaling_13, ref_scaling_93, ref_scaling_75} conclude that scaling consistently benefits runtime of the simplex method (and barrier method in the case of \cite{ref_scaling_13}). On the other hand \cite{ref_scaling_12} measures no benefit with respect to runtime or number of steps performed by the simplex method. All authors, however, seem to agree that scaling may reduce numerical problems encountered by the solver. Likewise, the authors of \cite{guidelines_klotz} explain the numerical difficulties solvers face when presented with a problem with large numeric range. They also find that these numerical problems often lead to performance degradation for state-of-the-art LP solvers. Similarly, the practical guides to both Gurobi \footnote{https://www.gurobi.com/documentation/9.0/refman/num\_tolerances\_and\_user\_sc.html} and GAMS \footnote{Bruce McCarl's GAMS Newsletter Number 41} suggest scaling input values in order to improve solver performance. 

% \subsection{Equilibration scaling}
% This simple scaling technique is reported to be effective for IPM in \cite{ref_scaling_13}. It maps all elements in $A$ and $b$ to values between $-1$ and $1$. It proceeds by first dividing each row $A_{i,.}, b_i$ by its maximum (in absolute value) and then doing the same for all columns $A_{., i}$ and $b$.

% \subsection{Bridge over troubled water: bringing best practice from operations research into energy system modelling }
% Questions:
% \begin{itemize}
% 	\item What do we know from operations research about this class of problems? \textit{text}
% 	\item What is Markowitz tolerance and why should I care when it has to be tightened? And this could be relevant somehow:
% 	"Warning: unscaled primal violation = 0.00537109 and residual = 0.00537109"
% 	Well-scaled models should take care of these things
% \end{itemize}
% \textit{Basically: what effects do the properties that we described above (large, sparse, bigM, ...) have on the various algorithms that we have available (simplex, primal-dual interior point, ...?).}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% previously existing content begins:

% Moreover, LPs corresponding to ESMs have the following properties:
% \begin{itemize} 
% \item Highly sparse matrices: problem formulations are highly sparse, before and after presolve, and thus simplex algorithms may be unsuitable. OR theory suggests that pivot methods are indeed unsuitable for this class of problem \mb{Add some reference or explanation here why this is the case}. However, using interior point methods does not lead to sparse solutions. You may end up with lots of very small fractional values. This is something discussed a lot in OR theory. But does it matter for us?
% \item Scaling issues: without manual intervention, problem formulations have large numerical ranges, potentially causing long solve times of, or sub-optimal solutions by interior point methods;
% \begin{itemize}
% 	\item Unmet demand BigM is also important here.
% \end{itemize}
% \item Degeneracy: Instability of solution time related to certain constraints: the solution time of Gurobi’s “crossover” is very sensitive to small model or parameter changes \mb{can we get an example of small parameter changes that affect crossover time?}.
% \end{itemize}

% Also, memory use is an issue. We monitor that and check whether there’s anything we can do about it.

% end
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

==> methods.tex <==


\section{Methods} \label{subsec_methods}
In the following we want to determine best practices when it comes to solving ESMs. 
In particular, we are interested in models generated by the Calliope modelling framework \cite{calliope} \mb{is this the correct thing to cite for calliope?} and how well these models can be solved using existing linear programming solvers. 
In the following paragraphs we formulate the questions we are interested in and how we want to answer them.

\paragraph{Algorithm Choice}
We compare the suitability of the two major classes of algorithms: Simplex methods and Barrier methods. As discussed in Section \ref{sec_solving_lp}, the barrier method run by itself returns a midface solution which is approximately optimal, whereas the simplex method returns a basic feasible solution. But the barrier method allows running a crossover method to find a BFS, taking the midface solution as start value. We thus consider running both the barrier method by itseld (barrier) and the barrier method with a subsequent run of crossover (barrier+crossover). 

For this discussion we consider two questions: (1) how fast does each method terminate, and (2) how "good" is the returned solution. To answer (1) we perform benchmarks for each of the solution methods and on several models. To answer (2) we first analyze the returned solution in terms of several relevant metrics: does the algorithm converge to a solution, what is the objective value, what is the fraction of non-zeros in the solution. In a second step, we perform several case studies where we analyze the semantic differences between midface and vertex solutions of concrete Calliope models.

\paragraph{Scaling} 
As discussed in Section \ref{sec_properties}, ESMs often have a large numeric range. We investigate if our models have the same problem and if it can be effectively mitigated using automatic scaling. To test this we benchmark the runtime of various models with and without scaling and quantify the effects of scaling. We consider each of the three algorithm classes for this.

\paragraph{Solver Choice}
We compare the suitability of the commercial Gurobi solver and the open-source Coin-OR solver for our problems. Again, this section relies mostly on runtime benchmarks.

\paragraph{Modelling Guidelines}
An interesting but difficult question is if there are semantic properties of ESMs that make the optimization problem inherently hard to solve and thus lead to bad solver performance. Here we perform some case studies on problematic Calliope models and show how these models can be "debugged".

\vspace{20pt}
We limit the scope of our investigations by explicitly excluding the following aspects
\begin{enumerate}
    \item We use the well-known solvers Gurobi and Coin-OR and their implementations of the standard Simplex and Barrier methods. We don't investigate specialized or custom solver implementations such as the network simplex method or the highly parallelizable instance of the barrier method developed in \cite{ref_parallel_ip}.
    \item All our model formulations are LPs or MILPs. We don't consider using other formalisms such as network flow.
    \item We run most of our experiments on a single (or a few) core(s) on standard hardware and we are not considering tuning the hardware to our workloads. 
\end{enumerate}

\subsection{Experimental Setup}
The input models used for the experiments are specified in table \ref{tab:models}
\begin{table}[h!]
    \centering
    \begin{tabular}{|l|l|}
    \hline
     Name & Model \\
     \hline
     Euro & 34-zone Euro-Calliope model\footnotemark with the manual scaling undone \\
     UK & 30-zone UK-Calliope\footnotemark \\
     Bangalore & 10-zone Bangalore-Calliope\footnotemark \\
     BangaloreLP & Same as Bangalore but without integrality constraints \\
     \hline
    \end{tabular}
    \caption{Calliope models used in experiments}
    \label{tab:models}
\end{table}
\footnotetext[1]{https://github.com/calliope-project/euro-calliope}
\footnotetext[2]{https://github.com/calliope-project/uk-calliope}
\footnotetext[3]{https://github.com/brynpickering/bangalore-calliope}

We will often add a postfix to model names to indicate the time range, e.g. Euro\_15d and Euro\_5m refer to the Euro-Calliope model run over a 15 day and a 5 months time range respectively.

The benchmarks were all performed on the Euler cluster of ETH Zürich. All experiments where runtimes were measured were performed on the same setup as summarized in table \ref{tab:hardware}. Each experiment was run alone on a full node, i.e. on 36 cores, to avoid competing processes from affecting the runtime. Note, however, that the number of cores does not correspond to the number of software threads. Except where explicitly noted we set the number of software threads to 4. 
\begin{table}[h!]
\centering
\begin{tabular}{|l|p{10.5cm}|}
\hline 
CPU model & Hardware specification \\
\hline 
XeonGold\_6150 & Two 18-core Intel Xeon Gold 6150 processors (2.7-3.7 GHz), 192 GB of DDR4 memory clocked at 2666 MHz \\
\hline
\end{tabular}
\caption{Hardware specification for benchmark runs}
\label{tab:hardware}
\end{table}

The authors of \cite{performance_variability} observe that the performance of MILP solvers is non-deterministic and is often subject to large variation due to seemingly unimportant changes: different machines, compilers, libraries can all lead to vastly different performance. We observe the same behaviour for Gurobi's LP solvers, mostly for the crossover phase (including final simplex cleanup). In order to account for this variability in our benchmarks, we perform each measurement several times only changing the random seed value of Gurobi. For each benchmark we indicate the number of repetitions, the average and min/max runtimes.


\subsection{Scaling Method}
In the following we discuss our implementation of \textit{autoscaling} that automatically scales Calliope models. As discussed in Section \ref{sec_scaling}, simply minimizing the condition number of the constraint matrix $A$, apart from being hard, may not be desirable (c.f. section 5 in \cite{ref_scaling_12}). \cite{ref_scaling_75} distinguishes between:
\begin{itemize}
    \item optimal scaling methods that minimize a certain metric on the constraint matrix $A$.
    \item empirical scaling methods, such as equilibration, that are sometimes found to work well in practice but don't provide any guarantees about their result
\end{itemize}
For optimal scaling methods \cite{ref_scaling_75} lists two possible objectives
\begin{align}
    d &:= \frac{\max_{i,j} A_{i,j}}{\min_{i,j} A_{i,j}} \label{eq_d}\\
    \sigma &:= \sum_{i,j} \log(|A_{i,j}|)^2 \label{eq_sigma}
\end{align}
There are algorithms that approximately solve both \ref{eq_d} \cite{algo_d} and \ref{eq_sigma} \cite{algo_sigma}. We devise our own approximation for \ref{eq_d} that incorporates additional domain knowledge about our models.

Most variables in Calliope are associated with some physical quantity such as energy or costs. \cite{beam_me} observe that it is common in ESMs that for example costs of technologies differ by many orders of magnitude (e.g. operational cost of roof-pv and investment cost of large thermal units). However, often times it happens that this effect is aggravated by representing physical quantities with standard units such as kWh and dollars regardless of the range of their values. Meaning that not only the ranges of values for quantities of the same unit are large but also there are large differences between different physical quantities. Informally, our approximation of $d$ automates this choice of unit for physical quantities. Let $U$ be the set of units in our model and $A_u$ the set of values in the model that have unit $u \in U$. Our goal is to find scaling factors $f_u$ for each unit $u \in U$ that minimize
\begin{equation} \label{eq_kappa}
\kappa' := \frac{\max_{u \in U} \max_{a \in A_u} f_u \cdot a}{\min_{v \in U} \min_{b \in A_v} f_v \cdot b}
\end{equation}
Note that changing the unit of a physical quantity is a special case of the scaling considered in Section \ref{sec_scaling} with $R = I$ and $S = \mathbf{diag}(f_{u_i})$ where $u_i$ for $i \in [n]$ is the unit of the i-th decision variable. 

In the following we first discuss some considerations when choosing scaling factors and then we explain how we actually compute them.

\paragraph{Choosing scaling factors that tamper with the precision of input values will corrupt the model}
In order to see the significance of numeric precision, consider the following example:
Consider the inequality $0.1 x \leq 100$. If we scale this inequality by $\frac{1}{3}$ we get the inequality $\frac{1}{30} x \leq \frac{100}{3}$. In mathematics the second inequality is equivalent to the first one, but in floating point arithmetic it is not. Let us assume for simplicity that we work in a decimal floating point system with $5$ decimal digits precision, then the second inequality becomes $0.03333 x \leq 33.33333$. Note that $100$ got scaled by $0.3333333$ and that $0.1$ got scaled only with $0.3333$. The inequality is thus no longer equivalent to the original inequality, in fact the second inequality now reduces to $x \leq 1000.0999$. Note that the relative error $\frac{1000.0999 - 1000}{1000}$ is exacly $\frac{0.3333333}{0.3333} - 1$. The relative error thus increases with the numeric range of the inequality. This loss of precision can be avoided if all scaling factors are chosen to be powers of $2$.

\paragraph{Optimal scaling factors may lead to prohibitively large or small values}
Gurobi recommends that all values in a model be between $10^{-3}$ and $10^6$ \footnote{ https://www.gurobi.com/documentation/9.0/refman/num\_advanced\_user\_scaling.html}. The absolute size of values matters to the solver because it internally uses absolute tolerances to compare values. In particular, having input values smaller than the solvers tolerances means that the solver can no longer distinguish between legitimate values and values arising from round-off errors \cite{guidelines_klotz}.
Ensuring that absolute values stay above a certain threshold sometimes limits how much $\kappa'$ can be decreased. Consider the following example:

Let $u$ and $v$ be the two base units in our model and let's assume that the derived units in our model all have the form $u$, $v$ or $\frac{u}{v}$. Assume the values in our model have the following ranges:
\begin{center} 
    \begin{tabular}{|l|r|r|}
    \hline 
         unit & min & max  \\
         \hline 
         $u$ & 1 & 50 \\
         $v$ & 0.001 & 100 \\
         $\frac{u}{v}$ & 0.001 & 100 \\
         \hline
    \end{tabular}
\end{center}
Here $\kappa' = 10^5$ cannot be decreased any further. Assume that we want to ensure that all values in our model have absolute value at least $0.01$. In order to achieve this we need to choose scaling factors $f_v \geq 10$ and $f_u \geq 10 \cdot f_v$. Thus after scaling it holds that $\kappa' \geq \frac{10 \cdot f_v \cdot 50}{f_v \cdot 0.001} = 5\cdot 10^5$ which is larger than the original $\kappa'$.

There is thus a tradeoff between minimizing $\kappa'$ and ensuring that the values have a sensible absolute size.

\paragraph{Computing optimal scaling factors}
Summarizing our previous findings we now want to compute scaling factors, one for each unit in the model, that 
\begin{itemize}
    \item Minimize $\kappa'$
    \item Are powers of $2$
    \item Don't scale absolute values of input data below some threshold
\end{itemize}
In the following we write \emph{unit} to mean the name of an abstract quantity such as \emph{energy} and not a concrete unit such as \emph{kWh}. We further distinguish between \emph{base units} and \emph{units}. The sets $U$ of \emph{base units} and $V$ of \emph{units} are related as follows:
\begin{align*}
    u \in U \Longrightarrow u \in V, \quad
    u \in U \Longrightarrow \frac{1}{u} \in V, \quad
    u_1, u_2 \in U \Longrightarrow \frac{u_1}{u_2} \in V
\end{align*}
This distinction is necessary because in our models we frequently encounter combinations of units such as \emph{cost per energy} and \emph{energy}. Scaling \emph{energy} by a factor $s$ we necessarily need to scale \emph{cost per energy} by the reciprocal $\frac{1}{s}$ in order to retain consistency. In other words when changing the unit of \emph{energy} from \emph{kWh} to \emph{Wh} we also need to change the unit of \emph{cost per energy} from $\frac{1}{\emph{kWh}}$ to $\frac{1}{\emph{Wh}}$. Let us also introduce a special unit $\textbf{1} \in U$ for all quantities that have no unit. All units $v \in V$ can now be represented as a fraction of base units $v = \frac{u_i}{u_j}$ \mb{variable cost\_energy\_cap\_per\_distance has unit cost/(energy*distance) so in order for the optimization to consider this variable, we would need to relax definition of unit}.

Note that all variables of column $i$ have the unit of the $i$-th decision variable. Thus denote by $u_i, v_i \in U$ for each $i \in [n]$ the base units satisfying that all variables in column $i$ of $A$ have unit $\frac{u_i}{v_i} \in V$. Moreover, let $S \subseteq \mathcal{R}^+$, $S = \{ f_u\ |\ u \in U \}$ be the set of scaling factors for each unit. We now want to find scaling factors for $u \in U$ that minimize $\kappa'$. More precisely we wish to solve
\begin{align*} 
\min_{S \subseteq \mathcal{R}^+} 
\max_{\substack{0 \leq i,j \leq m \\ 0 \leq k,l \leq n}} 
\frac{
    \frac{f_{u_k}}{f_{v_k}} 
    A_{i,k}
    }{
    \frac{f_{u_l}}{f_{v_l}} 
    A_{j,l}
} 
\end{align*}
We can rephrase this into an LP by taking logs of the entries of $A$ and of the scaling factors $s \in S$. 
\begin{align*} 
\min \quad &r \\
\text{s.t. } \forall\ i,j,k,l.\ &\log(f_{u_k}) - \log(f_{v_k}) + \log(A_{i,k}) \\
- &\log(f_{u_l}) + \log(f_{v_l}) - \log(A_{j,l}) \leq r
\end{align*}
We don't actually need to consider all entries of $A$. It suffices to include the minimum and the maximum of value of each unit. This simplification considerably reduces the amount of constraints from $n^2m^2$ to $|U|^2$ which is usually very small (below 100). 

As discussed above we additionally need to constrain $S$ to consist only powers of $2$ in order not to tamper with the input precision. This is equivalent to restricting $\log(f_u)$ to the integers for each unit $u \in U$. We do this by solving the relaxed LP and then rounding the scaling factors to the next integer.

Moreover, we need to restrict each scaling factor by an additional constraint that ensures that values are not scaled below a certain threshold.

% maybe exclude these paragraphs
%\paragraph{scaling leads to a different BFS}
%Theory: First, changing the model's geometry, it is possible to converge to an entirely different basic feasible solution BFS. Second, the optimality tolerances will cause scaled and unscaled models to run up to different relative distances to optimal BFS. \mb{third, same reasons as performance variability}
%Measurements: This happens consistently, even when choosing Gurobi's internal scaling we converge to a different solution. Note, that these solutions have the same objective value up to some tolerance, they simply have different values for the decision variables.

%\paragraph{The absolute value of scaling factors does not directly influence accurracy of result}
%Theory: accurracy of solution (i.e. $c^\intercal (x-x^*)$ as well as feasibility violations $\lVert b - Ax \rVert$ (for $Ax > b$) can be controlled by feasibilityTol and optimalityTol parameters. These are absolute values, thus scaling up $A, b, c$ will have the effect that $\lVert b - Ax \rVert$ and  $c^\intercal (x-x^*)$ gets scaled up and thus the algorithm has to do more work to be optimal/feasible.

%Measurements: Trying to measure this effect for barrier with crossover (i.e. basic solutions) by scaling up/down the scaling factors of the euro model didn't give consistent results: both scaling up and down sometimes increased precision and sometimes decreased precision.

%It seems the relationship between scaling factor size and the size of the \textit{relevant} values in the model is complicated and model dependant and we cannot generally predict the latter from the former. In particular, values with a unit composed of a fraction of two real base units won't be scaled differently at all. If the bulk of values has this kind of units, then absolute values of scaling factors won't have a large effect. Moreover, the tolerances only provide a range of precision within which the actual solution must fall, nothing prevents the solution from being better than this threshold. 
